From univariate to multivariate coupling between continuous signals and point processes: a mathematical framework

Time series datasets often contain heterogeneous signals, composed of both continuously changing quantities and discretely occurring events. The coupling between these measurements may provide insights into key underlying mechanisms of the systems under study. To better extract this information, we investigate the asymptotic statistical properties of coupling measures between continuous signals and point processes. We first introduce martingale stochastic integration theory as a mathematical model for a family of statistical quantities that include the Phase Locking Value, a classical coupling measure to characterize complex dynamics. Based on the martingale Central Limit Theorem, we can then derive the asymptotic Gaussian distribution of estimates of such coupling measure, that can be exploited for statistical testing. Second, based on multivariate extensions of this result and Random Matrix Theory, we establish a principled way to analyze the low rank coupling between a large number of point processes and continuous signals. For a null hypothesis of no coupling, we establish sufficient conditions for the empirical distribution of squared singular values of the matrix to converge, as the number of measured signals increases, to the well-known Marchenko-Pastur (MP) law, and the largest squared singular value converges to the upper end of the MPs support. This justifies a simple thresholding approach to assess the significance of multivariate coupling. Finally, we illustrate with simulations the relevance of our univariate and multivariate results in the context of neural time series, addressing how to reliably quantify the interplay between multi channel Local Field Potential signals and the spiking activity of a large population of neurons.

==> neuralComp_coro5proof_old.tex <==
% Proof of Corollary~\ref{corol:uniuncoupl_linearPhase}]
% \begin{proof}[Proof of Corollary~\ref{corol:uniuncoupl_linearPhase}]
\begin{proof}[Proof]
  % \michel{still minor rewriting to do for this proof (no need to take the limit of kappa, just write down the modified equation resulting from updating above proof)}
  Similar to Corollary~\ref{corol:kappaplv}, we can derive the asymptotic $\rm PLV$ (Eq.(\ref{eq:theoPLVhomoSPT})) for this case,
  from the definition in Eq.(\ref{thePLV}).
  We apply the intensity function $\lambda = \lambda_0$ in Corollary~\ref{corol:1DPLV}.
  The $\rm PLV$ asymptotic value ($\rm PLV^*$) can be derived simply
  by changing the integration variable from $mt$ to $\theta$.


  The covariance matrix of the asymptotic distribution,
  can be derived by the procedure we used for the proof of
  Corollary~\ref{corol:kappaplv}.
  We plug the constant rate $\lambda_0$ as $\lambda(t)$ in Corollary~\ref{corol:1DPLV}
  and integrate on $[0,\,T]$:
\begin{equation}
    \left(\rm Cov(Z) \right)_{11}
    = \frac{\lambda_0}{\Lambda(T)^2} \int_0^T \cos^2(\phi(t)) dt\,.
    % \label{covz11}
  \end{equation}
  As we assumed that $\phi(t)$ is a linear function of time (Assumption~\ref{assum:linearPhase})
  % (\ie $\tau'$ is constant everywhere)
  , we have:
  % (similar to Eq.(\ref{eq:simpSlope})), we have:
  \begin{equation}
    \left(\rm Cov(Z) \right)_{11}
     = \frac{\lambda_0}{\Lambda(T)^2} \int_0^T \cos^2(mt) dt\,. 
    % \label{covz11}
  \end{equation}
  We change  the integration variable from $mt$ to $u$,

  \begin{align}
    \left(\rm Cov(Z) \right)_{11}
    & = \frac{\lambda_0}{\Lambda(T)^2} \int_0^T \cos^2(mt) dt \\
    & = \frac{\lambda_0}{\Lambda(T)^2} \frac{1}{m} \int_0^{u(T)} \cos^2(u) du\\
    & = \frac{\lambda_0}{\Lambda(T)^2} \frac{1}{m} \frac{u(T)}{2}\\
    & = \frac{\lambda_0}{\Lambda(T)^2} \frac{1}{m} \frac{mT}{2}\,.
    % \label{covz11}
  \end{align}
  As $\Lambda(T) = \int_0^T \lambda_0 dt = \lambda_0T$,
  we have: 
  \begin{align}
    \left(\rm Cov(Z) \right)_{11}
    & = \frac{\lambda_0 T}{2\Lambda(T)^2}
     = \frac{\Lambda(T)}{2\Lambda(T)^2}
     = \frac{1}{2\Lambda(T)} \\
     & = \frac{1}{2\lambda_0 T}
    % \label{covz11}
  \end{align}
  We can also have a similar calculation for the imaginary part \ie $\left(\rm Cov(Z) \right)_{22}$.
  The off-diagonal elements of the covariance matrix vanish due to symmetry of integrand.

  Therefore, we showed that for the scaled residual,
  % estimated quantity $\widehat{\text{\rm PLV}}_K$
  % (note that $\rm PLV^* = 0$),
  \[
    Z =  \sqrt{K}\left(\widehat{\rm PLV}_K - \rm PLV^* \right)\,,
    \]
  converges to a zero mean isotropic complex Gaussian:
  \begin{equation*}
    \sqrt{K}\left(\widehat{\rm PLV}_K - \rm PLV^* \right)
    \underset{K\rightarrow +\infty
    }{\longrightarrow}\mathcal{N}\left(
      \left[\begin{matrix}
        0\\
        0
      \end{matrix}\right], \frac{1}{2 \lambda_0 T}\left[
      \begin{matrix}
        1&0\\
        0&	1
      \end{matrix}\right]\right)\,.
\end{equation*}
We also implicitly showed that,
    \[
    \lambda_0\exp(\kappa\cos(\phi(t)-\varphi_0)) \underset{\kappa\rightarrow 0
    }{\longrightarrow} \lambda_0 \,.
  \]

  
  Given that, $\rm PLV^* = 0$ (no coupling), estimated quantity $\widehat{\text{\rm PLV}}_K$
   is normally distributed asymptotically,
% Therefore, the covariance matrix resulting from Eq.(\ref{eq:covPLSPT}) with $\kappa = 0$,
  % is the asymptotic covariance of $\rm PLV$ residuals or $\rm PLV$ itself
  if  $[0,\,T]$ corresponds to an integer number of periods of the  oscillation, and
  if $\phi$ is a linear function of time.
  % Therefore, can get the 
  % to  homogeneous Poisson spike train cor
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "neuralComp"
%%% End:


==> neuralComp_coro_uniuncoupl_v0.tex <==
\begin{corol}
  \label{corol:uniuncoupl}
  Under the assumptions of Corollary~\ref{corol:1DPLV},
  we assume additionally that the point process is homogeneous Poisson with rate $\lambda_0 $
  and that $\phi(t)$ is strictly increasing (almost everywhere) and differentiable on $[0,\,T]$. 
   Let $\theta \mapsto \tau(\theta)$ be its inverse function (such that $\tau(\phi(t))=t$).
  Then the expectation of $\widehat{\mbox{PLV}}_K$ converges (for $K\mapsto +\infty$) to
   \begin{equation}
     \label{eq:theoPLVhomoSPT}
     \text{\rm PLV}^*=\frac{\int_{\phi(0)}^{\phi(T)} e^{\textbf{i}\theta}
       \tau'(\theta)d\theta}{\phi(T)-\phi(0)}\,.
     \end{equation}
  \shs{The previous form of eq \ref{eq:theoPLVhomoSPT} still exist in the tex file as a comment. I think the current form is compatible with previous corolary and less confusing for the reader}\michel{I put it back above, we need it to be able to assume homogeneity, which is the point of the corollary}
  \begin{equation}
    \label{eq:theoPLVhomoSPT}
    \text{\rm PLV}^*=\frac{\int_{\phi(0)}^{\phi(T)} e^{\textbf{i}\theta}
      d\theta}{\phi(T)-\phi(0)}\,.
  \end{equation}
  Additionally, if $\phi(T)-\phi(0)$ is a multiple of $2\pi$, \ie if $[0,\,T]$ corresponds to an integer number of periods of the oscillation, 
  and if $\phi(t)$ is linearly increasing, 
  then this expectation vanishes and the asymptotic covariance of $Z$ becomes
  \begin{equation}\label{eq:theoPLVhomoCov}
    \text{\rm Cov}
    \left[
      \begin{matrix}
        \text{Re}\{Z\}\\
        \text{Im}\{Z\}
      \end{matrix}
    \right]=\frac{1}{2 \lambda_0 (\phi(T)\!-\!\phi(0))}\left[
      \begin{matrix}
        1&0\\
        0&	1
      \end{matrix}\right]\,.
  \end{equation}
% \begin{equation}\label{eq:theoPLVhomoCov}
  %   \text{\rm Cov}
  % \left[
  % \begin{matrix}
  % \text{Re}\{Z\}\\
  % \text{Im}\{Z\}
  % \end{matrix}
  % \right]=\frac{1}{2 \lambda_0 \alphaT}\left[
  % \begin{matrix}
  % 1&0\\
  % 0&	1
  % \end{matrix}\right]\,.
  % \end{equation}
\end{corol}
\michel{modified to have homogenous process. modify proof and equations if needed}\michel{introduce covariance without extra assumption+potentially move the linear phase case as a remark after the coroll instead of inside it.}
% proof corol:uniuncoupl
% \begin{proof}[Sketch of the proof of corollary~\ref{corol:uniuncoupl}]
\begin{proof}[Sketch of the proof]
  The result stems from using the intensity function $\lambda_0 $ in Corollary~\ref{corol:1DPLV}.
  Then using change of variable in the integrals and exploiting the symmetries of the functions
  (see full proof in Appendix~\ref{app:proof}).
  % The result is straightforward by using $\kappa = 0$ as the coupling strength parameter
  % following the steps of the proof of Corollary~\ref{corol:kappaplv}.
\end{proof}
The first part of the corollary will be further illustrated in the next paragraphs. The second part of the corollary Eq.~(\ref{eq:theoPLVhomoCov})
guarantees an isotropic Gaussian PLV distribution under the null
hypothesis of no coupling. 
A similar isotropy result will be 
exploited in the multivariate case of Section~\nameref{sec:multiCoupl}.

%%% Local Variables:
%%% mode: latex
%%% End:

